Resource Efficient Mountainous Skyline Extraction using Shallow Learning

Skyline plays a pivotal role in mountainous visual geo-localization and localization/navigation of planetary rovers/UAVs and virtual/augmented reality applications. We present a novel mountainous skyline detection approach where we adapt a shallow learning approach to learn a set of filters to discriminate between edges belonging to sky-mountain boundary and others coming from different regions. Unlike earlier approaches, which either rely on extraction of explicit feature descriptors and their classification, or fine-tuning general scene parsing deep networks for sky segmentation, our approach learns linear filters based on local structure analysis. At test time, for every candidate edge pixel, a single filter is chosen from the set of learned filters based on pixel's structure tensor, and then applied to the patch around it. We then employ dynamic programming to solve the shortest path problem for the resultant multistage graph to get the sky-mountain boundary. The proposed approach is computationally faster than earlier methods while providing comparable performance and is more suitable for resource constrained platforms e.g., mobile devices, planetary rovers and UAVs. We compare our proposed approach against earlier skyline detection methods using four different data sets. Our code is available at \url{https://github.com/TouqeerAhmad/skyline_detection}.

==> space_crunch.tex <==
\makeatletter

\setlength\belowcaptionskip{6pt \@plus 4pt \@minus -6pt}
\setlength\abovecaptionskip{2pt}

% \long\def\@makecaption#1#2{
% \vspace*{\abovecaptionskip}
%    \setbox\@tempboxa\hbox{\small \noindent {\bf #1.}~{\it #2}}
%    \setlength{\@ctmp}{\hsize}
%    \addtolength{\@ctmp}{-\@figindent}\addtolength{\@ctmp}{-\@figindent}
%    % IF longer than one indented paragraph line
%    \ifdim \wd\@tempboxa >\@ctmp
%       % THEN DON'T set as an indented paragraph
%       {\small{\bf #1.}{~\it#2}\par}
%    \else
%       % ELSE center
%       \hbox to\hsize{\hfil\box\@tempboxa\hfil}
%   \fi\vspace*{\belowcaptionskip}}

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-1.2ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-.6ex \@plus -2ex \@minus -.2ex}%
                                   {.5ex \@plus.2ex}%
	                           {\normalfont\large\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-.5ex\@plus -.2ex \@minus -.2ex}%
                                     {.2ex \@plus .2ex}%
                                     {\normalfont\large\bfseries}}
\let\paragraph\textbf
\abovedisplayskip=4pt plus 3pt minus 6pt 
\abovedisplayshortskip=0pt plus 3pt 
\belowdisplayskip=6pt plus 3pt minus 6pt 
\belowdisplayshortskip=0pt plus 3pt minus 3pt 

\floatsep 4pt plus 2pt minus 2pt 
\textfloatsep 8pt plus 2pt minus 4pt
\intextsep 6pt plus 2pt minus 2pt  
\dblfloatsep 4pt plus 2pt minus 2pt 
\dbltextfloatsep 6pt plus 2pt minus 4pt 
\@fptop 2pt plus 1fil \@fpsep 6pt plus 2fil \@fpbot 0pt plus 1fil 
\@dblfptop 6pt plus 1fil \@dblfpsep 6pt plus 2fil \@dblfpbot 2pt plus 1fil


\makeatother

\def\closemath{
\abovedisplayskip=3pt plus 3pt minus 1pt 
\abovedisplayshortskip=0pt plus 1pt minus 1pt 
\belowdisplayskip=3pt plus 3pt minus 1pt 
\belowdisplayshortskip=0pt plus 1pt minus 1pt }

\def\tightmath{
\abovedisplayskip=4pt plus 2pt minus 1pt 
\abovedisplayshortskip=2pt plus 1pt minus 1pt 
\belowdisplayskip=4pt plus 2pt minus 1pt 
\belowdisplayshortskip=2pt plus 1pt minus 1pt }
\def\crushmath{
\abovedisplayskip=1pt plus 1pt minus 2pt 
\abovedisplayshortskip=1pt plus 1pt minus 2pt 
\belowdisplayskip=1pt plus 1pt minus 2pt 
\belowdisplayshortskip=1pt plus 1pt minus 2pt }
\tightmath

